Contrastive and Non-Contrastive Self-Supervised Learning Recover Global and Local Spectral Embedding Methods

Self-Supervised Learning (SSL) surmises that inputs and pairwise positive relationships are enough to learn meaningful representations. Although SSL has recently reached a milestone: outperforming supervised methods in many modalities\dots the theoretical foundations are limited, method-specific, and fail to provide principled design guidelines to practitioners. In this paper, we propose a unifying framework under the helm of spectral manifold learning to address those limitations. Through the course of this study, we will rigorously demonstrate that VICReg, SimCLR, BarlowTwins et al. correspond to eponymous spectral methods such as Laplacian Eigenmaps, Multidimensional Scaling et al. This unification will then allow us to obtain (i) the closed-form optimal representation for each method, (ii) the closed-form optimal network parameters in the linear regime for each method, (iii) the impact of the pairwise relations used during training on each of those quantities and on downstream task performances, and most importantly, (iv) the first theoretical bridge between contrastive and non-contrastive methods towards global and local spectral embedding methods respectively, hinting at the benefits and limitations of each. For example, (i) if the pairwise relation is aligned with the downstream task, any SSL method can be employed successfully and will recover the supervised method, but in the low data regime, VICReg's invariance hyper-parameter should be high; (ii) if the pairwise relation is misaligned with the downstream task, VICReg with small invariance hyper-parameter should be preferred over SimCLR or BarlowTwins.

==> chapter1.tex <==
% \documentclass{article}


% % if you need to pass options to natbib, use, e.g.:
% %     \PassOptionsToPackage{numbers, compress}{natbib}
% % before loading neurips_2022


% % ready for submission
% \usepackage[preprint]{neurips_2022}


% % to compile a preprint version, e.g., for submission to arXiv, add add the
% % [preprint] option:
% %     \usepackage[preprint]{neurips_2022}


% % to compile a camera-ready version, add the [final] option, e.g.:
% %     \usepackage[final]{neurips_2022}


% % to avoid loading the natbib package, add option nonatbib:
% %    \usepackage[nonatbib]{neurips_2022}


% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{xcolor}         % colors

% \input{math_commands}
% % if you use cleveref..
% \usepackage[capitalize]{cleveref}

% \title{A Spectral Theory of Deep Learning II:\\Amortized Spectral Analysis Enables Test-Time Prediction}


% % The \author macro works with any number of authors. There are two commands
% % used to separate the names and addresses of multiple authors: \And and \AND.
% %
% % Using \And between authors leaves it to LaTeX to determine where to break the
% % lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% % authors names on the first line, and the last on the second line, try using
% % \AND instead of \And before the third author name.


% \author{%
%   Randall Balestriero\\
%   Meta AI Research\\
%   NYC, USA\\
%   \texttt{rbalestriero@fb.com} \\
%   % examples of more authors
%   \And
%   Yann LeCun \\
%   Meta AI Research \& NYU\\
%   NYC, USA\\
%   \texttt{ylecun@fb.com} \\
%   % \AND
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
% }


% \begin{document}


% \maketitle


% \begin{abstract}
%   The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
%   both the left- and right-hand margins. Use 10~point type, with a vertical
%   spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
%   bold, and in point size 12. Two line spaces precede the abstract. The abstract
%   must be limited to one paragraph.
%   The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
%   both the left- and right-hand margins. Use 10~point type, with a vertical
%   spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
%   bold, and in point size 12. Two line spaces precede the abstract. The abstract
%   must be limited to one paragraph.The abstract
%   must be limited to one paragraph.
%   The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
%   both the left- and right-hand margins. Use 10~point type, with a vertical
%   spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
%   bold, and in point size 12. Two line spaces precede the abstract. The abstract
%   must be limited to one paragraph.
% \end{abstract}



% \input{content/introduction}
% \input{content/background}
% \input{content/vicreg_sup}
% \input{content/conclusion}

% \begin{enumerate}


% \item For all authors...
% \begin{enumerate}
%   \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
%     \answerTODO{}
%   \item Did you describe the limitations of your work?
%     \answerTODO{}
%   \item Did you discuss any potential negative societal impacts of your work?
%     \answerTODO{}
%   \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
%     \answerTODO{}
% \end{enumerate}


% \item If you are including theoretical results...
% \begin{enumerate}
%   \item Did you state the full set of assumptions of all theoretical results?
%     \answerTODO{}
%         \item Did you include complete proofs of all theoretical results?
%     \answerTODO{}
% \end{enumerate}


% \item If you ran experiments...
% \begin{enumerate}
%   \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
%     \answerTODO{}
%   \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
%     \answerTODO{}
%         \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
%     \answerTODO{}
%         \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
%     \answerTODO{}
% \end{enumerate}


% \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
% \begin{enumerate}
%   \item If your work uses existing assets, did you cite the creators?
%     \answerTODO{}
%   \item Did you mention the license of the assets?
%     \answerTODO{}
%   \item Did you include any new assets either in the supplemental material or as a URL?
%     \answerTODO{}
%   \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
%     \answerTODO{}
%   \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
%     \answerTODO{}
% \end{enumerate}


% \end{enumerate}


% \bibliography{iclr2022_conference}
% \bibliographystyle{plainnat}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \appendix


% \section{Proofs}
% \label{proof:section}

% \subsection{Proof of Var/Cov}
% \label{proof:var_cov}

% \begin{align*}
%     \|\mZ^T\mZ-\mI \|_F^2=\| \mV_z\mSigma^2\mV_z^T-\mI\|_F^2=\|\mSigma^2-\mI\|_F^2=\|\vsigma^2-\mathbf{1}\|_2^2
% \end{align*}

% \subsection{Proof of Optimal Matrix}
% \label{proof:optimal_matrix}


% \begin{align*}
%     \mZ^T\mY=\mZ^T\mZ\mW\iff &(U_{z}\Sigma_z V_z^{\top})^T\mY=(U_{z}\Sigma_z V_z^{\top})^\top(U_{z}\Sigma_z V_z^{\top})\mW\\
%     \iff &V_z\Sigma_z^TU_{z}^T\mY=V_z\Sigma_z^T \Sigma_z V_z^{\top}\mW\\
%     \iff &\mW^* \in \{ (V_z\Sigma^{-1}_zU_{z}^T+\tilde{V}_z\mM)\mY:\mM \in \mathbb{R}^{K \times C}\},
% \end{align*}

% \subsection{Proof of Recovery}
% \label{proof:recovery}

% \subsection{Proof of Optimal Value}
% \label{proof:optimal_value}


% \begin{align*}
%     V_z\Sigma_z^TU_{z}^T\mY=&V_z\Sigma_z^T \Sigma_z V_z^{\top}\mW^*\\
%     \implies  V_z\Sigma_z^TU_{z}^T\mY=&V_z\Sigma_z^T \Sigma_z V_z^{\top}(V_z\Sigma^{-1}_zU_{z}^T+\mM)\mY\\
%     \implies  V_z\Sigma_z^TU_{z}^T\mY=&V_z\Sigma_z^T \Sigma_z \Sigma^{-1}_zU_{z}^T\mY\\
%     \implies  V_z\Sigma_z^TU_{z}^T\mY=&V_z\diag(\sigma_z)^2 \Sigma^{-1}_zU_{z}^T\mY\\
%     \implies  V_z\Sigma_z^TU_{z}^T\mY=&V_z\Sigma_z^TU_{z}^T\mY
% \end{align*}
% where the last equality follows since $\diag(\sigma_z)^2 \Sigma^{-1}_z$ will either multiply $(\sigma_z)_i^2$ with $(\Sigma^{-1}_z)_{i,i}=\frac{1}{(\sigma_z)_i}$ if $(\sigma_z)_i$ is nonzero, and otherwise if $(\sigma_z)_i$ is $0$, then it will be the product between $0$ for $(\sigma_z)_i^2$ and $0$ for $(\Sigma^{-1}_z)_{i,i}$ giving back the original value for $(\sigma_z)_i$.

% \subsection{Proof of Loss Derivation}
% \label{proof:loss_value}

% \begin{align*}
%     \frac{1}{2}\|\mY -\mZ \mW^* \|_{F}^2=&\frac{1}{2}\|\mY -\mZ (V_z\Sigma^{-1}_zU_{z}^T+\tilde{V}_z\mM)\mY \|_{F}^2\\
%     =&\frac{1}{2}\|\mY -U_{z}\Sigma_z V_z^{\top} V_z\Sigma^{-1}_zU_{z}^T\mY \|_{F}^2\\
%     =&\frac{1}{2}\|\mY -U_{z}\Sigma_z\Sigma^{-1}_zU_{z}^T\mY \|_{F}^2\\
%     =&\frac{1}{2}\|(\mI -U_{z}\Sigma_z\Sigma^{-1}_zU_{z}^T)\mY \|_{F}^2\\
%     =&\frac{1}{2}\|(U_{z}U_{z}^T -U_{z}\Sigma_z\Sigma^{-1}_zU_{z}^T)\mY \|_{F}^2\\
%     =&\frac{1}{2}\|(\mI -\Sigma_z\Sigma^{-1}_z)U_{z}^T\mY \|_{F}^2\\
%     =&\frac{1}{2}\|\mY \|_{F}^2-\frac{1}{2}\|\Sigma_z\Sigma^{-1}_zU_{z}^T\mY \|_{F}^2\\
%     =&\frac{1}{2}\|\mY \|_{F}^2-\frac{1}{2}\|\Sigma_z\Sigma^{-1}_zU_{z}^T\mU_{y}\Sigma_y \|_{F}^2\\
%     =&\frac{1}{2}\|\mY \|_{F}^2-\frac{1}{2}\sum_{i,j}1_{\{(\sigma_z)_i>0\}}\langle (\mU_z)_i,(\mU_y)_j\rangle^2(\sigma_y)^2_j,
% \end{align*}


% \subsection{Proof of VICReg Recovering Laplacian Eigenmaps (\cref{thm:vicreg_main})}
% \label{proof:vicreg_main}


% Our goal now is to show that whenever the VICReg loss is minimized, with the correct data-augmentation i.e. the exact pairwise relationship between points, then the representation provided by VICReg is optimal i.e. it can be used to minimized the training error with true labels. To do so, we start from \cref{eq:VICReg} and turn the invariance term as a Dirichlet Energy on a given graph as in 
% \begin{align}
% \mathcal{L}_{\rm vic}=&\alpha \sum_{k=1}^{K}\max\hspace{-0.05cm}\left(0,1-\sqrt{\Cov(\mZ)_{k,k}}\right) \hspace{-0.08cm}+ \beta\hspace{-0.05cm} \sum_{j=1,j\not = k}^{K}\Cov(\mZ)^2_{k,j}+\gamma\sum_{i=1}^{N}\sum_{j=1}^{N}\mW_{i,j}\|\mZ_{j,.}-\mZ_{i,.}\|_2^2\nonumber \\
%   =&\alpha \sum_{k=1}^{K}\max\hspace{-0.05cm}\left(0,1-\sqrt{\Cov(\mZ)_{k,k}}\right)\hspace{-0.08cm}+ \beta \sum_{j=1,j\not = k}^{K}\Cov(\mZ)^2_{k,j}+2\gamma\underbrace{\Tr\left(\mZ^T\mL\mZ\right)}_{\text{Dirichlet Energy}},\label{eq:vicreg2}
% \end{align}
% with $\mW_{i,j}=\mW_{j,i}=c\iff \exists n \text{ s.t. } (i,j)\in\mathcal{P}_n,\forall i,j \in \{1,\dots,N\}^2$, and with $\mL\triangleq \mD-\mW$ the Laplacian matrix of the graph where $\mD$ is the degree matrix with $0$ entries everywhere except for the diagonal with $(\mD)_{i,i}=\sum_{j}(\mW) _{i,j}$. The equality in \cref{eq:vicreg2} follows from
% \begin{align*}
%     \Tr\left(\mZ^T\mL\mZ\right)=&\sum_{d}(\mZ^T\mL\mZ)_{d,d}=\sum_{i,j}\mL_{i,j}\langle (\mZ)_{j,.}.(\mZ)_{i,.}\rangle\\
%     =&\sum_{i}\|(\mZ)_{i,.} \|_2^2(\mD)_{i,i}-\sum_{i,j}(\mW)_{i,j}\langle (\mZ)_{j,.}.(\mZ)_{i,.}\rangle\\
%     =&\frac{\sum_{i}\|(\mZ)_{i,.} \|_2^2(\mD)_{i,i}+\sum_{i}\|(\mZ)_{i,.} \|_2^2(\mD)_{i,i}}{2}-\sum_{i,j}(\mW)_{i,j}\langle (\mZ)_{j,.}.(\mZ)_{i,.}\rangle\\
%     =&\frac{\sum_{i}\sum_{j}\|(\mZ)_{i,.} \|_2^2(\mW)_{i,j}+\sum_{i}\sum_{j}\|(\mZ)_{i,.} \|_2^2(\mW)_{i,j}}{2}-\sum_{i,j}(\mW)_{i,j}\langle (\mZ)_{j,.},(\mZ)_{i,.}\rangle\\
%     =&\frac{1}{2}\sum_{i}\sum_{j}(\mW)_{i,j}\|(\mZ)_{i,.}-(\mZ)_{j,.}\|_2^2,
% \end{align*}
% which is a famous derivation in graph signal processing relating pairwise distances to Dirichlet energy of the underlying graph with Laplacian $\mL$. Using $\alpha>0$ and $\beta>0$ and assuming that we ought to find a representation $\mZ$ that minimizes the VICReg loss means that $\Cov(\mZ)=(\mZ-\mu)^T(\mZ-\mu)=\mZ^T\mZ+\mu\mu^T$ and thus, due to the covariance regularization, implies that $\mu=\mathbf{0}$. Hence, we have that $\Cov(\mZ)$ is a diagonal matrix with diagonal entries great or equal to $1$ as in  $\Cov(\mZ)=\mZ^T\mZ=\diag(\vt)$ with $(\vt)_i\geq 1$. 


% Up until this point, we did not leverage any assumption. Without loss of generality, we will now assume that $\mZ^T\mZ=\mI$ (see \cite{liang2021generalizing} for the general case that extends our following derivations). In that case, and under minimized variance and covariance term is equivalent to the following simplified Brockett \cite{brockett1991dynamical} optimization problem
% \begin{align*}
%     \min_{\mZ^T\mZ=\mI} \Tr(\mZ^T\mL\mZ),
% \end{align*}
% which is minimized (see Corollary 4.3.39 from \url{https://anandinstitute.org/pdf/Roger_A.Horn.%20_Matrix_Analysis_2nd_edition(BookSee.org).pdf}
% ) for $\mZ$ to have as columns the eigenvectors associated to the smallest eigenvalues of $\mL$. Recalling that $\mL=\mI-\mG\mG^T$ we thus have that the columns of $\mZ$ are the left-singular vectors of $\mG$ associated with the greatest singular vectors. In fact, the eigenvectors of $\mG\mG^T$ are the left-singular vectors of $\mG$, and the eigenvectors of $I-\mG\mG^T$ and $\mG\mG^T$ are the same but with associated eigenvalue being $(1-\lambda^2)$.

% \subsection{Proof of Laplacian Eigenmap and VICReg (\cref{thm:vicreg_le})}
% \label{proof:vicreg_le}
% the proof is basically already done above.


% \subsection{Linear VICReg is LPP  (\cref{thm:vicreg_linear})}
% \label{proof:vicreg_lpp}

% \subsection{Linear VICReg with supervised relation matrix is LDA (\cref{thm:vicreg_linear})}
% \label{proof:vicreg_lda}


% The objective in 2-class LDA (see \citet{li2014fisher} for examples) is to minimize the following objective
% \begin{align*}
%     \max\frac{\va^T\mC_{b}\va}{\va^T\mC_{w}\va},
% \end{align*}
% where $\mC_{t}=\mX^T\mX,\mC_{w}=\mX^T(\mI-\mH)\mX,\mC_{b}=\mX^T\mH\mX$ encode the total/within/between cluster variances respectively using the supervised relation matrix $\mG$ from \cref{eq:H}.

% To DERIVATIONS OF THE ABOVE HERE


% Hence noticing that $H$ is a projection matrix i.e. $H^2=H$. the multi class problem can thus be formulated to be
% \begin{align*}
%     \max_{\mV}\frac{|\mV^T\mSigma_{b}\mV |}{| \mV^T\mSigma_{w}\mV|},
% \end{align*}
% which is known as the Fisher criterion. Whenever $\mSigma_{w}$ is invertible (if not, then the original data can be projected to a lower dimensional subspace without loss on information that would ensure that $\mSigma_{w}$ is invertible) then Fisher’s criterion is maximized leading to $\mV$ being the solution to the generalized eigenvalue problem
% \begin{align*}
%     \mV^*=&\argmax \frac{|\mV^T\mSigma_{b}\mV |}{| \mV^T\mSigma_{w}\mV|} 
%     =\text{solution to: } \mSigma_{b}\mV=\diag(\lambda) \mSigma_{w}\mV\\
%     =&\text{top eigenvectors of: } (\mSigma_{w})^{-1}\mSigma_{b}.
% \end{align*}
% Notice that the generalized eigenvalue problem is exactly
% \begin{align*}
%     \mX^T\mH\mX\mV=\diag(\lambda)\mX^T(\mI-\mH)\mX\mV,
% \end{align*}
% and that $\mH \mathbf{1}=\mathbf{1}$ we observe that this is exactly the same solution than the LPP problem with $\mH$ being the relation matrix and $\mI$ being the degree matrix of the graph. Hence we obtain that LPP is equivalent to LDA whenever one uses the supervised relation matrix $\mH$ as $\mG$ (which was first pointed out in \cite{kokiopoulou2011trace}) and that it corresponds exactly to VICReg in the linear regime (as per \cref{proof:vicreg_lpp}). We also note that the eigenvalue of the above matrix $(\mSigma_{w})^{-1}\mSigma_{b}$ might seem to be arbitrary. However we have the following lemma that ensure that the eigenvalues of are real nonnegative.

% \begin{lemma}
% \label{lemma:NN}
% The eigenvalues of $(\mSigma_{w})^{-1}\mSigma_{b}$ are equal to the eigenvalues of $\mSigma_{w}^{-1/2}\mSigma_{b}\mSigma_{w}^{-1/2}$ which is symmetric hence all are nonegative and real.
% \end{lemma}





% \subsection{SimCLR Exact Loss Minimization}
% \label{proof:simclr_discussion}

% Do the iterative procedure, iterate between finding the closest CR1 matrix and closest NN matrix until convergence , \dots


% \subsection{Proof of SimCLR \cref{thm:simclr}}
% \label{proof:simclr}


% The SimCLR loss is given by
% \begin{align*}
%     -\sum_{i,j}(\mG)_{i,j}(\mS(\mZ))_{i,j}=-\Tr(\mG^T\mS(\mZ))=-\Tr(\mG\mS(\mZ)),
% \end{align*}
% which we can minimize with respect to $\mS$. In fact, for now we will assume that $\mZ$ can be tuned such that any similarity matrix $\mS$ can be recovered from $\mZ$. Using a similar approach as done in the VICReg case, and using the fact that $\mS$ is symmetric semidefinite positive, hence can always be expressed as $\mS=\mU_s \mSigma_s\mU_s^T$ we have that 
% \begin{align*}
%     \min_{\mS:\|\mS\|^2_F=c}-\Tr(\mG\mS)=&\min_{\mU:\mU^T\mU=\mI,\sigma:\|\sigma\|_2^2=c}-\Tr(\mG^T\mU \mSigma\mU^T)\\
%     =&\max_{\mU:\mU^T\mU=\mI,\sigma:\|\sigma\|_2^2=c}\Tr(\mU^T\mG\mU \mSigma)\\
%     =&\max_{\mU:\mU^T\mU=\mI,\sigma:\|\sigma\|_2^2=c}\Tr(\mU^T\mU_g\mSigma_g\mU^T_g\mU \mSigma),
% \end{align*}
% o find an upper bound for the maximum, apply the Von-Neumann trace inequality. In particular, we have 
% \begin{align*}
%     \max_{\mU:\mU^T\mU=\mI,\sigma:\|\sigma\|_2^2=c}\Tr(\mU^T\mU_g\mSigma_g\mU^T_g\mU \mSigma)&\leq \sum_{n=1}^{N}\lambda_n(\mSigma_g\mU^T_g\mU \mSigma)\\
%     &\leq \sum_{n=1}^{N}(\mSigma_g)_{n,n}\lambda_n(\mU^T_g\mU \mSigma),
% \end{align*}

% leading to $\mSigma=\diag(\mU^T\mG^T\mU)c/\|\diag(\mU^T\mG^T\mU)\|_2$

% In supervised learning one is given with not only the input samples $\mX^{(o)}$ but also associated target values $\mY \in \mathbb{R}^{N^{(o)}\times K}$. 

% In this setting, the supervised mean squared error loss is given by $
%     \mathcal{L} = \frac{1}{N^{(o)}}\sum_{n=1}^{N^{(o)}}\|\mY_n -\mZ_n \|_2^2$ and 
% which, after some derivations provided in \cref{sec:derivation}, can be expressed as
% \begin{align}
%     \mathcal{L} =& \frac{1}{C}\sum_{c=1}^{C}\bigg\|\vy_c -\frac{ 1}{|\mathcal{P}_c|}\sum_{n \in \mathcal{P}_{c}}\mZ_n \bigg\|_2^2+ \sum_{i=1}^{N^{(o)}}\sum_{j=1}^{N^{(o)}}\mW_{i,j}\|\mZ_n -\mZ_m \|_2^2\nonumber \\
%     =&
%     \frac{1}{C}\sum_{c=1}^{C}\bigg\|\vy_c - \frac{1}{|\mathcal{P}_c|}\sum_{n \in \mathcal{P}_{c}} \mZ_n  \bigg\|_2^2+\Tr\left(\mZ^T\mL\mZ\right),\label{eq:supervised}
% \end{align}
% where $C$ is the number of classes i.e. number of distinct rows in $\mY$ given by $\vy_1,\dots,\vy_C$ and $\mathcal{P}_{c}$ gives the indices of the rows in $\mY$ where $\vy_c$ is repeated, with $\mW_{i,j}=\mW_{j,i}=1/(|\mathcal{P}_c| (|\mathcal{P}_c|-1))\iff \exists c \text{ s.t. } (i,j)\in\mathcal{P}_c,\forall i,j \in \{1,\dots,N\}^2$, and with $\mL\triangleq \mD-\mW$ the Laplacian matrix of the graph where $\mD$ is the degree matrix, in our case each diagonal entry is $1/C$. 



% \subsection{Proof of BarlowTwins in the Linear Regime (\cref{thm:BT_cca})}
% \label{proof:BT_cca}


% The tie between CCA and LDA is not new. In fact, if one considers one dataset to be the samples and the other to be the class labels (binary variables for two-class problems or a variation of one-hot encoding for multi-class problems) then CCA and LDA are equivalent \citep{bartlett1938further,hastie1995penalized}. We we demonstrate here is that this is also the case when the views are both obtained from samples, but with different matching, exactly fitting the BarlowTwins family of losses.

% Considering that $\mG$ has degree $1$ and that all the entries are either $0$ or a constant such that similar inputs are normalized by the cardinality of their group. In short, it follows the same structure than \cref{eq:H} except that it is constructed as desired, not necessarily from labels. In that scenario, it is quite clear that the cross-covariance $\mC_{\rm lr}$ is obtained (assuming for clarity that the inputs have $0$ mean) by $\mZ^T_{\rm left}\mZ_{\rm right}=\mZ^T\mG\mZ$ since
% \begin{align*}
%     \frac{1}{N}\mZ^T\mG\mZ=& \frac{1}{N}\sum_{c=1}^{C}\sum_{i \in \mathcal{N}_c}\sum_{j \in \mathcal{N}_c}\frac{1}{N_c}\vz_i\vz_j^T\\
%     =& \frac{1}{N}\sum_{c=1}^{C}N_c\sum_{i \in \mathcal{N}_c}\sum_{j \in \mathcal{N}_c}\frac{1}{N_c^2}\vz_i\vz_j^T\\
%     =& \frac{1}{N}\sum_{c=1}^{C}N_c\frac{\sum_{i \in \mathcal{N}_c}\vz_i}{N_c}\frac{\sum_{j \in \mathcal{N}_c}\vz_j^T}{N_c}\\
%     =& \sum_{c=1}^{C}\frac{N_c}{N}\mu_c \mu_c^T=\mS_{B},
% \end{align*}
% recovering the between (inter-cluster) variance. Now, since we have that $\mS_{T}=\mS_{B}+\mS_{W}$ we directly have that $\mS_{W}=\frac{1}{N}\left(\mZ^T\mZ-\mZ^T\mG\mZ\right)=\frac{1}{N}\left(\mZ^T\left(\mI-\mG\right)\mZ\right)$




% Given the usual pairwise relationship between samples in $\mZ$ described in $\mG$, we obtain that matching two positive pairs is equivalent to $\mZ^T\mG\mZ$ since $\mG$ is basically a permutation matrix that will switch the rows of $\mZ$ to form $\mG\mZ$, and then matching those with the original $\mZ^T$ produce the cross-covariance. 



% The whole point of CCA is to find the two inputs that most correlate when mapped to two matrices. We will see below how to characterize those vectors and quantify the amount of produces correlation from the spectrum of the two linear transformations. However, this is only useful if we wanted to learn a transformation of the input that does that. In our case, we want to measure how good is a given representation $\mZ$. Hence, we need instead to find $\mZ$ for which those vectors are equal. 


% Note that we could remove the duplicates but since those will become a constant we keep them. We thus have realization $a$ which is from $\mZ$ and realization $b$ which is from $\mG\mZ$. the corresponding covariance are thus
% We obtain \begin{align*}
%     &C_{aa}=\mZ^T\mZ,\\
%     &C_{ab}=\mZ^T\mG\mZ,\\
%     &C_{ba}=\mZ^T\mG\mZ,\\
%     &C_{bb}=\mZ^T\mZ,
% \end{align*}
% since we have that $\mG=\mG^T$ and $\mG^2=\mI$. Using the result from 
% CCA \cite{uurtio2017tutorial} we have the the CCA is equal to the sum of the singular values of $C_{bb}^{-1}C_{ba}C^{-1}_{aa}C_{ab}$ which corresponds to $\Tr((\mZ^T\mZ)^{-1}\mZ^T\mG\mZ)$ since $C_{ab}=C_{ba}$ and $C_{aa}=C_{bb}$. This further simplifies into $\Tr(\mZ^\dagger\mG\mZ)$. Using Von Neumann’s trace inequality \cite{von1937some} we have that 
% \begin{align*}
%     CCA = \Tr(\mZ^\dagger\mG\mZ) \leq \sum_{n=1}^{N}(\vsigma_{zz^\dagger})_n(\vsigma_{g})_n,
% \end{align*}
% we see that for $CCA$ to reach that upper bound, one must have the top left singular vectors of $\mG$ as the left singular vectors of $\mZ$ since
% \begin{align*}
%     \Tr(\mZ^\dagger\mG\mZ)=&\Tr((\mV\mSigma^T\mU^T\mU\mSigma\mV^T)^{-1}\mV\mSigma^T\mU^T\mG\mU\mSigma\mV^T)\\
%     =&\Tr((\mV\mSigma^T\mSigma\mV^T)^{-1}\mV\mSigma^T\mU^T\mG\mU\mSigma\mV^T)\\
%     =&\Tr(\mV(\mSigma^T\mSigma)^{-1}\mV^T\mV\mSigma^T\mU^T\mG\mU\mSigma\mV^T)\\
%     =&\Tr(\mSigma(\mSigma^T\mSigma)^{-1}\mSigma^T\mU^T\mG\mU),
% \end{align*}
% where $\mSigma(\mSigma^T\mSigma)^{-1}\mSigma^T$ is a diagonal $N \times N$ matrix with entries that are $1$ for the first $K$ entries, and $0$ afterward. Hence, the above is maximized for any matrix $\mZ$ whose top left singular vectors are any rotation of the top left singular vectors of $\mG$.

% Also, \cite{healy1957rotation,ewerbring1989canonical} have shown that using the SVD one could solve CCA as follows.

% Also good ref \cite{hardoon2004canonical}

% {\bf Recover LDA from supervised CCA (BarlowTwins).}~To recover this result, we closely follow the methodology from \citet{kursun2011canonical}. First, notice that the CCA optimum solves the following eigenvalue problem
% \begin{align*}
%     \mC_{ll}^{-1}\mC_{lr}\mC_{rr}^{-1}\mC_{rl}\vu_{\rm CCA}=\lambda_{\rm CCA} \vu_{\rm CCA},
% \end{align*}
% but noticing that in our case $\mX_{\rm l}$ and $\mX_{\rm r}$ are permutations of each other, we directly obtain that
% \begin{align*}
%     \mC_{ll}^{-1}\mC_{lr}\mC_{rr}^{-1}\mC_{rl}\vu_{\rm CCA}=\lambda_{\rm CCA} \vu_{\rm CCA}
%     \iff\mS_{T}^{-1}\mS_{B}\mS_{T}^{-1}\mS_{B}\vu_{\rm CCA}=\lambda_{\rm CCA} \vu_{\rm CCA},
% \end{align*}
% now starting from the LDA loss, we will see that we recover the CCA one thanks to the above facts
% \begin{align*}
%     \mS_{B}\vu_{\rm LDA}=&\lambda_{\rm LDA}\mS_{W} \vu_{\rm LDA} &&\text{(original LDA parameter)}\\
%     \iff\mS_{B}\vu_{\rm LDA}=&\lambda_{\rm LDA}(\mS_{T}-\mS_{B}) \vu_{\rm LDA}\\
%     \iff\mS_{B}(1+\lambda_{\rm LDA})\vu_{\rm LDA}=&\lambda_{\rm LDA}\mS_{T} \vu_{\rm LDA}\\
%     \iff\mS_{B}\vu_{\rm LDA}=&\frac{\lambda_{\rm LDA}}{(1+\lambda_{\rm LDA})}\mS_{T} \vu_{\rm LDA}\\
%     \iff(\mS_{T})^{-1}\mS_{B}\vu_{\rm LDA}=&\frac{\lambda_{\rm LDA}}{(1+\lambda_{\rm LDA})} \vu_{\rm LDA}\\
%     \iff(\mS_{T})^{-1}\mS_{B}(\mS_{T})^{-1}\mS_{B}\vu_{\rm LDA}=&(\frac{\lambda_{\rm LDA}}{(1+\lambda_{\rm LDA})})^2 \vu_{\rm LDA}&&\text{(original CCA problem)}
% \end{align*}
% hence given the LDA or CCA solutions one can recover the others, the only different is the singular values, which can also be found from each other. Also, recall that the eigenvalues are real positive as per \cref{lemma:NN}.




% \subsection{Proof of VICReg Optimality (\cref{thm:optimal_vicreg})}
% \label{proof:optimal_vicreg}

% The proof first uses \cref{thm:vicreg_le} that demonstrates how the optimal representation $\mZ$ will have the left singular vectors of $\mG$ up to rotations for the ones with multiplicity greater than one. Then, using that, we obtain from \cref{thm:optimal} that if those singular vectors are able to span the left singular vectors of $\mY$ then there exists a linear probe that will solve the task at hand, giving the desired result.


% \section{DeepCluster}
% \label{sec:deepcluster}
% \begin{theorem}
% DeepCluster is optimal as long as the mock $\mY$ has same left-singular vectors than the true $\mY$ which itself is true iff $\mZ$ has the same left-singular vectors than $\mY$.
% \end{theorem}

% K-means as orthogonal NMF \cite{ding2005equivalence,ding2006orthogonal}



% SVD to initialize NMF \cite{qiao2015new}

% K-means with PCA \cite{ding2004k}
% \end{document}
% CCA \cite{uurtio2017tutorial}

==> content/old_EM.tex <==
\section{JEM: A Simple Recipe To Include Self-Supervision In Any Latent Variable Probabilistic Model}


tighter is not better \citep{rainforth2018tighter}.





\subsection{JEM: The Joint-Expectation Maximization Algorithm}


We now suppose that we have a priori knowledge on the {\em positive relationship} between different samples. For example, $\vx_i$ and $\vx_j$ are semantically equivalent but originate from two different recording devices, views, or any other possible factor of variation. For a given sample index $i$, we denote by $N_i$ the set of indices of the semantically equivalent samples. Note that for some, we can have $N_i = \{i\}$ i.e. there are no other known equivalent sample.

We introduce SESAM which consists of a generalization of the ELBO. Starting with the same derivation as in the ELBO case of \ref{} we derive
% \begin{align*}
%     \log(p_{\theta}(\vx_n))=&\int q_{\gamma}(\vz)\log\left(\frac{p_{\theta}(\vx_n,\vz)}{q_{\gamma}(\vz|\vx_{N^{(i)}_1})}\prod_{j=1}^{|N^{(i)}|-1}\frac{q_{\gamma}(\vz|\vx_{N^{(i)}_{j}})}{q_{\gamma}(\vz|\vx_{N^{(i)}_{j+1}})}\times \frac{q_{\gamma}(\vz|\vx_{N^{(i)}_{-1}})}{p_{\theta}(\vz|\vx_n)}\right) d \vz\\
%     =&\underbrace{\mathbb{E}_{q_{\gamma}(\vz)}\left[p_{\theta}(\vx_n,\vz)\right]+\mathbb{H}(q_{\gamma}(\vz))}_{\text{Variational Lower Bound (ELBO)}}+\underbrace{\mathbb{K}\mathbb{L}(q_{\gamma}(\vz)||p_{\theta}(\vz|\vx_n))}_{\text{Bound tightness}},
% \end{align*}
for any nonnegative sum-to-one weight vector $\boldsymbol{\alpha}_{n} \in \Delta (|\mathcal{T}|)$ we have
\begin{align*}
    \log(p_{\theta}(\vx_n))
    =&\sum_{i=1}^{|\mathcal{T}|}\alpha_{n,i}\left(\mathbb{E}_{q_{\gamma}(\vz|_it(\vx_n))}\left[\log(p_{\theta}(\vx_n|\vz))\right]+\mathbb{K}\mathbb{L}(q_{\gamma}(\vz|t_i(\vx_n))||p_{\theta}(\vz))+\mathbb{K}\mathbb{L}(q_{\gamma}(\vz|t_i(\vx_n))||p_{\theta}(\vz|\vx_n))\right)\\
    &\geq \sum_{i=1}^{|\mathcal{T}|} \alpha_{n,i}\left(\mathbb{E}_{q_{\gamma}(\vz|t_i(\vx_n))}\left[\log(p_{\theta}(\vx_n|\vz))\right]+\mathbb{K}\mathbb{L}(q_{\gamma}(\vz|t_i(\vx_n))||p_{\theta}(\vz))\right),\;\;\text{(J-ELBO)}
\end{align*}

{\bf The J-ELBO can be as good, and even tighter than the ELBO.}

The lower-bound can also be tight, as the ELBO. In fact, we can quantify exactly the bound-tightness between the ELBO and the J-ELBO as
\begin{align}
    |\mathbb{K}\mathbb{L}(q_{\gamma}(\vz|\vx_n)||p_{\theta}(\vz|\vx_n))-\sum_{t \in \mathcal{T}}\frac{[\boldsymbol{\alpha}_n]_t}{|\mathcal{T}|}\mathbb{K}\mathbb{L}(q_{\gamma}(\vz|t(\vx_n))||p_{\theta}(\vz|\vx_n))|.
\end{align}
From the above, it is easy to see that as long as the identity mapping belongs to the space of transformations ${\rm identity} \in \mathcal{T}$, and that the weighting parameters $\boldsymbol{\alpha}_n$ are learnable, J-ELBO can only improve the log-likelihood estimate that was provided by the ELBO. We formalize this results below.


\begin{proposition}
If the identity mapping is present in the considered set of transformations, the J-ELBO can only be equal or tighter than the ELBO, as in 
$${\rm identity} \in \mathcal{T} \implies \exists \boldsymbol{\alpha}_{n} \in \Delta (|\mathcal{T}|) : \text{J-ELBO} \geq \text{ELBO},\forall \vx_n$$
\end{proposition}



with $\alpha_{i,.} \in \Delta (|N_i|)$ i.e. $\sum_{m \in N_i} \alpha_{i,m}=1$ and $\alpha_{i,m}\geq 0, \forall i,m$. For example taking $\alpha_{i,m}=1_{\{i=m\}}$ makes SESAM fall back to the ELBO. As a result, the only difference between traditional EM and ours, is that you simply need to weight a few losses together and then do maximization step on that.

ALGORITHM HOW PORTING EM -> JEM


\subsection{Walk-Through Examples}


\begin{itemize}
    \item GMM
    \item FA
    \item PPCA
    \item mixture + FA
    \item mixture + PPCA
\end{itemize}


\section{Empirical Validations}

\begin{itemize}
    \item MNIST/MedicalMNIST/CIFAR/...
    \item UCI
    \item Genomic data?
\end{itemize}


\section{Exploring The Natural Semantic Relationship Learned by Graphical Models}

Let's consider a VAE. What people have been doing is basically look at the nearest neighbour of $\vx_n$ in latent space i.e. search over $m \not = n$ for $d(f_{\mu}(\vx_n),f_{\mu}(\vx_n))$ where $d$ is usually the $\ell_2$ distance or cosine distance. This has a limitation which is that it only takes into account the symmetries learned by the encoder i.e. the amortized posterior. Although this should align with the generator mapping underlying symmetries, there is, in general, no guarantee. Hence this type of distance fails to provide the complete PGM understanding of a sample. Instead, we propose to use
\begin{align*}
    &d(\mathbb{E}_{q_{\gamma}(\vz|\vx_n)}\left[\log(p_{\theta}(\vx_n,\vz))\right]+\mathbb{H}(q_{\gamma}(\vz|\vx_m)),\mathbb{E}_{q_{\gamma}(\vz|\vx_m)}\left[\log(p_{\theta}(\vx_n,\vz))\right]+\mathbb{H}(q_{\gamma}(\vz|\vx_m)))
\end{align*}



\newpage
\newpage




\section{The Underlying Model of Self-Supervised Joint Embedding}

Consider the following data modeling distribution 
\begin{align*}
    &\begin{array}{l}
         \vz \sim \mathcal{N}(0,\sigma_{z}\mI)  \\
         \vh | \vz,c \sim \mathcal{N}(\mW\vz+\mu_c,\sigma_{z}\mI) 
    \end{array}&&\text{(Mixture of PPCA in latent space)}
    \\
    &\vx | \vh \sim \mathcal{N}(f_{\theta}(\vh),\sigma_{x}\mI),&&\text{(nonlinear generative process)}.\\
\end{align*}
we have the following posterior
\begin{align*}
    &\vz | \vh,c \sim \mathcal{N}\left(\left(\frac{\sigma_{h}}{\sigma_{z}}\mI+\mW\mW^T\right)^{-1}\mW^T(\vh-\mu_c),(\sigma_{z}^{-1}+\sigma_{h}^{-1}\mW\mW^T)^{-1}\right),&&\text{(projector)}.\\
    &\vh | \vx \sim \mathcal{N}(E_{\mu}(\vx_n)E_{\emSigma}(\vx_n)),&&\text{(backbone)}.\\
\end{align*}

{\bf Core model:} In the latent space, factors of variations are disentangled (translations/rotations now move along linear subspaces given by $\mW$, around each original image given by $\mu_c$).

That corresponds to a Gaussian Mixture Model with Gaussian prior on the cluster centers
\begin{align*}
    p_{\theta}(\mX,\mH,\mZ,\vc)=&p_{\theta}(\mX|\mH)p_{\theta}(\mH|\mZ,\vc)p_{\theta}(\mZ)p_{\theta}(\vc)
\end{align*}
with
\begin{align}
    \mX \triangleq \begin{bmatrix}
    \vx_1^T\\
    \dots \\
    \vx_N^T\\
    \end{bmatrix},
    \mH \triangleq \begin{bmatrix}
    \vh_1^T\\
    \dots \\
    \vh_N^T\\
    \end{bmatrix},
    \mZ \triangleq \begin{bmatrix}
    \vz_1^T\\
    \dots \\
    \vz_K^T\\
    \end{bmatrix},
    \vc\triangleq \begin{bmatrix}
    c_1\\
    \dots \\
    c_N^T\\
    \end{bmatrix},
\end{align}
where $K$ is the dataset size, and $N$ is equal to $K \times P$ where $P$ is the number of samples augmentations for each datum. Without loss of generality we consider $P$ to be the same for each datum. The complete likelihood is given by
\begin{align*}
    p_{\theta}(\mX,\mH,\mZ,\vc)=&\prod_{n=1}^{N}\mathcal{N}(\vx_n;D_{\theta}(\vh),\emSigma_{\vx})\prod_{k=1}^{C}\mathcal{N}(\vh_n;\mW\vz_k,\emSigma_{k})^{1_{\{c_n=k\}}}\prod_{k=1}^{C}\mathcal{N}(\vz_k;\mu_k,I)
\end{align*}
For now, we consider that we observe both $\mX$ and $\vc$ i.e. we observe the input samples and the cluster assignments through the augmented samples i.e. positive pairs. The true posterior $p_{\theta}(\mH,\mZ|\mX,\vc)$ is not tractable, we will resort of Variational-EM. But prior to that, we shall notice that the complete likelihood can be simplied. In fact, recalling Sec.~2.3.3 from \footnote{\url{https://www.microsoft.com/en-us/research/uploads/prod/2006/01/Bishop-Pattern-Recognition-and-Machine-Learning-2006.pdf}}, we obtain that
\begin{align*}
    p_{\theta}(\vh_n|c_n)\sim \mathcal{N}(\mu_{c_n},\sigma_{h}\mI+\sigma_{z}\mW\mW^T).
\end{align*}
Using a variational distribution for the unobserved variables as $q_{\phi}(\mH)\sim  \mathcal{N}(E_{\mu}(\vx),E_{\emSigma}(\vx))$
we obtain
\begin{align*}
    \log p_{\theta}(\vx_n) \geq&\mathbb{E}_{q_{\phi}(\mH)}\left[\log(p_{\theta}(\mX,\mH|\vc))\right]-\mathbb{E}_{q_{\phi}(\mH)}\left[\log(q_{\phi}(\mH))\right]+\log(p_{\theta}(\vc))&&\text{(ELBO)}\\
    =&\mathbb{E}_{q_{\phi}(\mH)}\left[\log(p_{\theta}(\mX|\mH))\right]+\mathbb{E}_{q_{\phi}(\mH)}\left[\log(p_{\theta}(\mH|\vc))\right]-\mathbb{E}_{q_{\phi}(\mH)}\left[\log(q_{\phi}(\mH))\right]+\log(p_{\theta}(\vc))\\
    =&\mathbb{E}_{q_{\phi}(\mH)}\left[\log(p_{\theta}(\mX|\mH))\right]-KL(q_{\phi}(\mH)||p_{\theta}(\mH|\vc))+\log(p_{\theta}(\vc))\\
    =&-\frac{1}{2\sigma_{x}}\|\vx_n-f_{\theta}(\vh_n)\|_2^2-\frac{1}{2}\Big[\log\left(\frac{|\sigma_h\mI+\sigma_{z}\mW\mW^T|}{|E_{\emSigma}(\vx_n)|}\right)-k\\
    &+(E_{\mu}(\vx_n)-\mu_c)^T(\sigma_h\mI+\sigma_{z}\mW\mW^T)^{-1}(E_{\mu}(\vx_n)-\mu_c)+tr((\sigma_h\mI+\sigma_{z}\mW\mW^T)^{-1}E_{\emSigma}(\vx_n)) \Big].
\end{align*}
with $\vh_n \sim q_{\phi}(\mH)$. Now we can see that the optimum for $\mu_c$ is given by $\frac{1}{|N_c|}\sum_{n \in N_c}E_{\mu}(\vx_n)$ which leads to
\begin{align*}
    \frac{1}{|N|}\sum_{n \in N}\log p_{\theta}(\vx_n) =&-\frac{D}{2}\log(2\pi \sigma_x)+\frac{k}{2}-\frac{1}{2\sigma_{x}|N|}\sum_{n \in N}\|\vx_n-f_{\theta}(\vh_n)\|_2^2-\frac{1}{2}\log\left(|\sigma_h\mI+\sigma_{z}\mW\mW^T|\right)\\
    &+\frac{1}{2}\log\left(|E_{\emSigma}(\vx_n)|\right)-\frac{1}{|N|}\sum_{c}\frac{1}{4|N_c|}\sum_{i,j \in N_c^2}\|E_{\mu}(\vx_i)-E_{\mu}(\vx_j)\|^2_{(\sigma_h\mI+\sigma_{z}\mW\mW^T)^{-1}}\\
    &-\frac{1}{2}tr((\sigma_h\mI+\sigma_{z}\mW\mW^T)^{-1}E_{\emSigma}(\vx_n))
\end{align*}









Hence, we choose a variational distribution for the unobserved variables that factorizes as $q_{\phi}(\mH,\mZ)=q_{\phi}(\mH)q_{\phi}(\mZ|\mH)$ with
\begin{align*}
    &q_{\phi}(\vh|\vx)\sim \mathcal{N}(E_{\mu}(\vx),E_{\emSigma}(\vx)),&&\text{(backbone)}\\
    &q_{\phi}(\vz|\vh)\sim \mathcal{N}(\mA\vh+\vb,\mL),&&\text{(projector/expander)}
\end{align*}
leading to the ELBO objective to be maximized
\begin{align*}
    \log p_{\theta}(\vx_n) \geq&\mathbb{E}_{q_{\phi}(\mH,\mZ)}\left[\log(p_{\theta}(\mX,\mH,\mZ,\vc))\right]-\mathbb{E}_{q_{\phi}(\mH,\mZ)}\left[\log(q_{\phi}(\mH,\mZ))\right]&&\text{(ELBO)}\\
    =&\mathbb{E}_{q_{\phi}(\mH)}\left[\log(p_{\theta}(\mX|\mH))\right]+\mathbb{E}_{q_{\phi}(\mH,\mZ)}\left[\log(p_{\theta}(\mH,\mZ,\vc))\right]-\mathbb{E}_{q_{\phi}(\mH,\mZ)}\left[\log(q_{\phi}(\mH,\mZ))\right]\\
    =&\mathbb{E}_{q_{\phi}(\mH)}\left[\log(p_{\theta}(\mX|\mH))\right]-KL(q_{\phi}(\mH,\mZ)||p_{\theta}(\mH,\mZ|\vc))+\log(p_{\theta}(\vc)).
\end{align*}
Crucial to our derivation is the fact that both $q_{\phi}(\mH,\mZ)$ and $p_{\theta}(\mH,\mZ|\vc)$ joint distributions can be expressed as Gaussians. In fact, using the fact we have
\begin{align*}
    &q_{\phi}(\mH,\mZ)\sim \mathcal{N}\left(
    \begin{pmatrix}
    E_{\mu}(\vx_n)\\
    \mA E_{\mu}(\vx_n)+\vb
    \end{pmatrix},\begin{pmatrix}
    E_{\emSigma}(\vx_n)&E_{\emSigma}(\vx_n)\mA^T\\
    \mA E_{\emSigma}(\vx_n)&\mL+\mA E_{\emSigma}(\vx_n)\mA^T
    \end{pmatrix}
    \right),\\
    &p_{\theta}(\mH,\mZ|\vc)\sim \mathcal{N}\left(
    \begin{pmatrix}
    \mW\mu_c\\
    \mu_c
    \end{pmatrix},\begin{pmatrix}
    \emSigma_c+\mW\mW^T&\mW\\
    \mW^T&I
    \end{pmatrix}
    \right)
\end{align*}
,
hence the KL divergence  $KL(q_{\phi}(\mH,\mZ)||p_{\theta}(\mH,\mZ|\vc))$ is known analytically as a function of the above means and covariances. The left-side expectation is approximated using the usual Monte-Carlo sampling.

\begin{align*}
    KL(\mathcal{N}(\mu_1,\emSigma_1)||\mathcal{N}(\mu_2,\emSigma_2))=\frac{1}{2}\left[\log\left(\frac{|\emSigma_2|}{|\emSigma_1|}\right)-k+(\mu_1-\mu_2)^T\emSigma_2^{-1}(\mu_1-\mu_2)+tr(\emSigma_2^{-1}\emSigma_1)\right]
\end{align*}
Using the fact that $det(\emSigma_2)=det(\emSigma_c+\mW\mW^T-\mW\mW^T)det(I)=det(\emSigma_c)$ and $det(\emSigma_1)=det(E_{\emSigma}(\vx)-E_{\emSigma}(\vx)\mA^T(\mL+\mA E_{\emSigma}(\vx_n)\mA^T)^{-1}\mA E_{\emSigma}(\vx))det(\mL+\mA E_{\emSigma}(\vx_n)\mA^T)$ and that 

\begin{align*}
    (\mu_1-\mu_2)^T\emSigma_2^{-1}(\mu_1-\mu_2)=&\|E_{\mu}(\vx_n)-\mW\mu_c-\mW(\mA E_{\mu}(\vx_n)+\vb-\mu_c)\|^2_{\emSigma_c}+ \|\mA E_{\mu}(\vx_n)+\vb-\mu_c \|_2^2\\
    =&\underbrace{\|E_{\mu}(\vx_n)-\mW(\mA E_{\mu}(\vx_n)+\vb)\|^2_{\emSigma_c}}_{\text{projector AE error}}+ \|\mA E_{\mu}(\vx_n)+\vb-\mu_c \|_2^2
\end{align*}
see \footnote{\url{https://people.eecs.berkeley.edu/~jordan/courses/260-spring10/other-readings/chapter13.pdf}}

\begin{proposition}
The projector/expander inference process corresponds to the one of probabilistic PCA when $\mL=\epsilon I$ and to the one of Factor Analysis when $\mL=diag(\epsilon)$.
\end{proposition}


The above justifies the use of the Eigendecomposition of $\mH$ as weight of $\mW$ as commonly used in many papers.
x

\newpage 

\newpage

by now using a one-sample estimate of $q_{\phi}(\mH)$ sampled from $\mathcal{N}(E(\mX),I)$ we obtain
\begin{align*}
    \log p_{\theta}(\vx_n) \approx&\log(p_{\theta}(\mX|H))-KL(q_{\phi}(H,\mZ)||p_{\theta}(H,\mZ|\vc))+\log(p_{\theta}(\vc))\\
    =&\log(p_{\theta}(\mX|H))-q_{\phi}(H)KL(q_{\phi}(\mZ|H)||p_{\theta}(H,\mZ|\vc))+\log(p_{\theta}(\vc))
\end{align*}

where we will use as usual the one-sample Monte-Carlo estimate of the expectation based on sampling of the learned variational posterior, and the reparametriztion trick to learn the variational posterior with gradient descent. Also let's say that we observe $c_n$ and that $p_{\theta}(c)$ is uninformative, we thus have
\begin{align*}
    \log p_{\theta}(\vx_n) \geq\mathbb{E}_{q_{\phi}(\vz|\vx_n)}\left[\log(p_{\theta}(\vx_n,\vz,c_n))\right]-D_{KL}(q_{\phi}(\vz|\vx_n,c_n)||p_{\theta}(\vz)),
\end{align*}


Using a Gaussian prior for $p_{\theta}$ and for the variational distribution, we have that 
\begin{align*}
    D_{KL}(q_{\phi}(\vz|\vx_n,c_n)||p_{\theta}(\vz))=\frac{1}{2}\left[\mu_{c_n}(\vx_n)^T\mu_{c_n}(\vx_n)+Tr(\emSigma_{c_n}(\vx_n))-k-\log(det(\emSigma_{c_n}(\vx_n)))\right],
\end{align*}
and
\begin{align*}
    \mathbb{E}_{q_{\phi}(\vz|\vx_n)}\left[\log(p_{\theta}(\vx_n,\vz,c_n))\right]\approx& \log(p_{\theta}(\vx_n|\vz_n))+\log(p_{\theta}(\vz_n))\\
    =&-\sum_{k=1}^{C}\sum_{n \in N_k}\frac{1}{2}\|\vx_n-\vz(\vx_n,c_n)\|_2^2+
\end{align*}
with $\vz_n \sim \mathcal{N}(\mu(\vx_n),\emSigma(\vx_n))$.



We will take $\log q_{\phi}(\vz|\vx_n) = \log \mathcal{N}(\vz; \mu_n, \emSigma_n)$ where the mean and covariance of the approximate posterior, $\mu_n$ and $\emSigma_n$, are outputs of the encoding
DN, i.e. nonlinear functions of datapoint $\vx_n$ from the variational parameters $\phi$.

Consider a simple case of
\begin{align*}
    p(\vx,\theta,c)=\kappa\prod_{k=1}^{C}\left(e^{-\frac{1}{2}\|\vx-\exp(\mG \theta)\mu_k\|_2^2}\right)^{1_{\{c=k\}}}p(\theta)
\end{align*}
\begin{align*}
    \log(\mathcal{L}(\vx))\leq& \mathbb{E}_{\theta,c|\vx}\left[\log(p(\vx,\theta,c))\right]\\
    =& \int \sum_{c=1}^{C}q(\theta,c|\vx)\log(p(\vx,\theta,c))d\theta\\
    =&-\frac{1}{2}\sum_{k=1}^{C}\int q(\theta,c=k|\vx)\|\vx-\exp(\mG \theta)\mu_k\|_2^2d\theta \\
    =&-\frac{1}{2}\sum_{k=1}^{C}\int \frac{q(\vx|\theta,c=k)}{\sum_{k=1}^{C}q(\vx|\theta,c=k)}\|\vx-\exp(\mG \theta)\mu_k\|_2^2d\theta
\end{align*}
\begin{enumerate}
    \item If $q$ is the true posterior $\implies$ EM-training 
    \item If $q$ is a variational distribution, add an Entropy regularization to also learn $q$ $\implies$ variational-EM
    \item if e.g. $c$ is observed, we obtain partially observed EM \dots
\end{enumerate}
\begin{align*}
    \log(\mathcal{L}(\sX))=&-\frac{1}{2}\sum_{n=1}^{N}\int q(\vx_n|\theta,c_n)\|\vx_n-\mM(\theta)\mu_c\|_2^2d\theta\\
    =&-\frac{1}{2}\sum_{n=1}^{N}\int q(\vx_n|\theta,c_n)\|\mM(\theta)(\mM(\theta)^{\dagger}\vx_n-\mu_c)\|_2^2+\|\mQ(\theta)\mQ(\theta)^{\dagger}\vx_n\|_2^2d\theta%\\
    % =&-\frac{1}{2}\sum_{n=1}^{N}\int e^{-\|\vx_n-\exp(\mG \theta)\mu_{c_n}\|_2^2}\|\vx_n-\exp(\mG \theta)\mu_{c_n}\|_2^2d\theta\\
    % =&-\frac{1}{2}\sum_{k=1}^{C}\sum_{n \in N_k}\int e^{-\|\vx_{n}-\exp(\mG \theta)\mu_k\|_2^2}\|\vx_{n}-\exp(\mG \theta)\mu_k\|_2^2d\theta\\
    % =&-\frac{1}{2}\sum_{n=1}^{N}\int q(\vx|\theta,c_n)\|\exp(\mG \theta)\vx_n-\exp(\mG \theta)\vx_m\|_2^2d\theta
\end{align*}


\begin{align*}
    \|\vx_n-\mM(\theta)\mu_c\|_2^2=&\|\mM(\theta)\mM(\theta)^{\dagger}\vx_n+\mQ(\theta)\mQ(\theta)^{\dagger}\vx_n-\mM(\theta)\mu_c\|_2^2\\
    =&\|\mM(\theta)(\mM(\theta)^{\dagger}\vx_n-\mu_c)+\mQ(\theta)\mQ(\theta)^{\dagger}\vx_n\|_2^2\\
    =&\|\mM(\theta)(\mM(\theta)^{\dagger}\vx_n-\mu_c)\|_2^2+\|\mQ(\theta)\mQ(\theta)^{\dagger}\vx_n\|_2^2\\
    &+2 (\mM(\theta)^{\dagger}\vx_n-\mu_c)^T\mM(\theta)^T\mQ(\theta)\mQ(\theta)^{\dagger}\vx_n\\
    =&\|\mM(\theta)(\mM(\theta)^{\dagger}\vx_n-\mu_c)\|_2^2+\|\mQ(\theta)\mQ(\theta)^{\dagger}\vx_n\|_2^2\\
    =&\|\mM(\theta)(\mM(\theta)^{\dagger}\vx_n-\mM(\theta')^{\dagger}\vx_m-\mQ(\theta')^{\dagger}\vx_m)\|_2^2+\|\mQ(\theta)\mQ(\theta)^{\dagger}\vx_n\|_2^2\\
    =&\|\mM(\theta)(\mM(\theta)^{\dagger}\vx_n-\mM(\theta')^{\dagger}\vx_m\|_2^2+\|\mM(\theta)\mQ(\theta')^{\dagger}\vx_m\|_2^2+\|\mQ(\theta)\mQ(\theta)^{\dagger}\vx_n\|_2^2\\
    &-2(\mM(\theta)(\mM(\theta)^{\dagger}\vx_n-\mM(\theta')^{\dagger}\vx_m))^T\mM(\theta)\mQ(\theta')^{\dagger}\vx_m\\
    =&\|\mM(\theta)(\mM(\theta)^{\dagger}\vx_n-\mM(\theta')^{\dagger}\vx_m\|_2^2+\|\mM(\theta)\mQ(\theta')^{\dagger}\vx_m\|_2^2+\|\mQ(\theta)\mQ(\theta)^{\dagger}\vx_n\|_2^2\\
    &-2\vx_n^T(\mM(\theta)^{\dagger})^T\mM(\theta)^T\mM(\theta)\mQ(\theta')^{\dagger}\vx_m-2\vx_m^T(\mM(\theta')^{\dagger})^T\mM(\theta)^T\mM(\theta)\mQ(\theta')^{\dagger}\vx_m\\
    =&\|\mM(\theta)(\mM(\theta)^{\dagger}\vx_n-\mM(\theta')^{\dagger}\vx_m\|_2^2+\|\mM(\theta)\mQ(\theta')^{\dagger}\vx_m\|_2^2+\|\mQ(\theta)\mQ(\theta)^{\dagger}\vx_n\|_2^2\\
    &-2\vx_n^T\mM(\theta)\mQ(\theta')^{\dagger}\vx_m-2\vx_m^T(\mM(\theta')^{\dagger})^T\mM(\theta)^T\mM(\theta)\mQ(\theta')^{\dagger}\vx_m
\end{align*}
\begin{align*}
    \log(\mathcal{L}(\sX))=&-\frac{1}{2}\sum_{n=1}^{N}\int e^{-\|\mM^{(t)}(\theta)(\mM^{(t)}(\theta)^{\dagger}\vx_n-\mu_c)\|_2^2-\|\mQ^{(t)}(\theta)\mQ^{(t)}(\theta)^{\dagger}\vx_n\|_2^2}(\|\mM(\theta)(\mM(\theta)^{\dagger}\vx_n-\mu_c)\|_2^2+\|\mQ(\theta)\mQ(\theta)^{\dagger}\vx_n\|_2^2)d\theta\\
    =&-\frac{1}{2}\sum_{n=1}^{N}\int\kappa(\theta)(\|\mM(\theta)(\mM(\theta)^{\dagger}\vx_n-\mu_c)\|_2^2+\|\mQ(\theta)\mQ(\theta)^{\dagger}\vx_n\|_2^2)d\theta\\
    =&-\frac{1}{2}\sum_{n=1}^{N}\int\kappa(\theta)(\|(\mM(\theta)^{\dagger}\vx_n-\mu_c)\|_{\mM(\theta)^T\mM(\theta)}^2+\vx_n^T(\mQ(\theta)^{\dagger})^T\mQ(\theta)^{\dagger}\vx_n ) d\theta\\
\end{align*}



\section{Measuring Information Content of Datasets?}

Let's consider the following definition of information content hold by a dataset as 
\begin{equation}
    IC(\sX)=\frac{\bigcup_{n=1}^{N}\vol(\mathcal{N}(\vx_n,I\epsilon))}{\vol(\mathcal{N}(\mu,\emSigma)}
\end{equation}
for a dataset with mean $\mu$ and covariance $\emSigma$.

==> content/risefall.tex <==
\section{Unifying Contrastive and Non-Contrastive Self-Supervised Methods with Graph Signal Processing}


The goal of Self-Supervised Learning (SSL) --- regardless of the training method --- is akin to unsupervised learning: to produce parsimonious latent representations $f_{\theta}(\vx)$ of observable signals $\vx$ that perform well on a variety of downstream tasks, in general employing a Deep Network (DN) as $f_{\theta}$. From that objective stem two major classes of SSL methods: contrastive and non-contrastive. Our goal in the first \cref{sec:unifying} is to cast and unify those two approaches under a Graph Signal Processing (GSP) form. From this, we will be able to identify the limitations of each formulation in \cref{sec:limitations}; to finally propose a novel Non-Contrastive method in the next \cref{sec:novel}.


\subsection{Casting Contrastive and Non-Contrastive Methods as Learning Signals on Graphs and Graph Laplacians}
\label{sec:unifying}



\textit{The goal of \textbf{Contrastive SSL} is to produce signals $f_{\theta}(\vx_n)$ such that the graph for which this signal is smooth is equal a known graph.} 


Let's first define the minimization problem that given a set of signals, gives the most likely graph
\begin{align}
    W_{d,\mathcal{R}}(\mX,\theta)=\argmin_{W \in \mathcal{W}}\sum_{i,j}d(f_{\theta}(\vx_i),f_{\theta}(\vx_j))W_{i,j}+\mathcal{R}(W),
\end{align}
with $\mathcal{W}$ the space of considered matrices. In general, $\mathcal{W}$ consists of symmetric matrices with nonnegative entries and zero-diagonal. If $W$ needs to be stochastic, then $\mathcal{W}$ also constrains the sum of each row to be equal to $1$. Hence $W_{d,\mathcal{R}}(\mX,\theta)$ is the graph ---expressed as a weight matrix--- for which $f_{\theta}(\mX)$ is smooth.
Let's denote the target graph given a batch of samples as $W^*(\mX)$, the contrastive loss thus takes the general form
\begin{align*}
    \theta^*_{\rm NC}=\min_{\theta} \ell\left(W^*(\mX),W_{d,\mathcal{R}}(\mX,\theta)\right),
\end{align*}

\begin{proposition}
Setting $\mathcal{R}(\mW)=\tau \sum_{i\not =j}(\log(\mW_{i,j})-1)$ with $\tau$ the temperature parameter (see \cref{fig:regularization1}), $d(\vu,\vv)=1-\frac{\langle \vu,\vv\rangle}{\|\vu\|_2 \|\vv\|_2}$ the cosine distance, $\mathcal{W}$ the space of stochastic matrices, and $\ell$ the cross-entropy (between stochastic matrices) recovers SimCLR.
\end{proposition}


Quickly, it has become clear that using the known relation from $W^*(\mX)$ could be suboptimal. For example, high amplitude data augmentation might make two inputs completely unrelated, similarly, another input in the mini-batch can be a better fit for different samples. Hence, emerged the idea to add a learning component to $W^*(\mX)$ as follows
\begin{align}
    W^*_{{\rm knn},d}(\mX,\theta)=\argmin_{W \in \mathcal{W}_{\rm knn}}\sum_{i,j}d(f_{\theta}(\vx_i),f_{\theta}(\vx_j))W_{i,j},
\end{align}
with $\mathcal{W}_{\rm knn}$ the space of weight matrices with binary entries and such that each row sums to $k$
\begin{align}
    \mathcal{W}_{\rm knn} \triangleq \left\{\sum_{n=1}^{N}\sum_{k\in \sB_k}\ve_n\ve_k^T+\ve_k\ve_n^T, \sB_n \in \mathcal{S}_{K}(N\setminus\{n\}),n=1,\dots,N \right\}
\end{align}

\begin{figure}[t!]
    \centering
    \begin{minipage}{0.5\linewidth}
    \includegraphics[width=\linewidth]{figures/regularization_gsp_1.png}
    \end{minipage}
    \begin{minipage}{0.45\linewidth}
    \caption{Caption}
    \label{fig:regularization1}
    \end{minipage}
\end{figure}

To recover the most prominent methods, set $\mathcal{R}(\mW)$ to be $\tau \sum_{i\not =j}(\log(\mW_{i,j})-1)$ with $\tau$ the temperature parameter with behavior depicted in \cref{fig:regularization1}, $d$ to be the cosine distance, and $\mathcal{W}$ to be the space of stochastic matrices, $\ell$ to be the cross-entropy (between stochastic matrices) and we recover exactly most of the contrastive methods by setting
\begin{align*}
    &W^*(\mX) \text{ is $0$ everywhere except for DA pairs}, &&\text{(SimCLR)}\\
    &W^*(\mX) \text{ is 1-NN graph}, &&\text{(NNCLR)}\\
    &W^*(\mX) \text{ is k-NN graph}, &&\text{(WeanSHIFT)}\\
    &W^*(\mX) \text{ is k-means graph}, &&\text{(DINO)}
\end{align*}

\textit{The goal of \textbf{Non-Contrastive Learning} is to produce signals $f_{\theta}(\vx_n)$ that are smooth with respect to a given graph structure, and that are non-degenerate.}


Hence, the non-contrastive loss takes the general form
\begin{align*}
    \theta^*_{\rm C}=\min_{\theta}\underbrace{\mathcal{R}(f_{\theta}(\mX))}_{\text{prevent collapse of the signal}}+\underbrace{\sum_{i,j}d(f_{\theta}(\vx_i),f_{\theta}(\vx_j))W^*_{i,j}(\mX)}_{\text{smoothness of the signal on the graph}}.
\end{align*}

For example taking $d$ to be the Euclidean distance, $W^*$ to be the same as in SimCLR, and $\mathcal{R}(f_{\theta}(\mX))=\|f_{\theta}(\mX)^Tf_{\theta}(\mX)-\mI\|_F^2$ leads to VICReg, or using $\log(\det(f_{\theta}(\mX)^Tf_{\theta}(\mX)))$ leads to TCR.



\begin{align*}
    \theta^*_{\rm C}=\min_{\theta}\underbrace{\mathcal{R}(f_{\theta}(\mX))}_{\text{prevent collapse of the signal}}+\min_{\mW \in \mathcal{W}}\underbrace{\sum_{i,j}d(f_{\theta}(\vx_i),f_{\theta}(\vx_j))W^*_{i,j}(\mX)}_{\text{smoothness of the signal on the graph}}.
\end{align*}


\subsection{Making VICReg a constrastive method}





\subsection{The Limitations of Each Method}
\label{sec:limitations}


The main limitation of contrastive method lies in the requirement to specify the connection between all pairs of nodes, and on the signals $\vh$ which overall must be at least of rank greater or equal to their dimensions.

batch sizeembedding size which must be at least the same as 










\subsection{deepCluster}

\begin{align}
    \mathcal{W}_{\rm Kmeans} \triangleq \left\{\sum_{\pi\in\Pi}\sum_{(i,j)\in\pi^2,i\not = j}\ve_i\ve_j^T+\ve_j\ve_i^T ,\forall \; \Pi \in \sB_{0,K,N} \right\}
\end{align}
with $\sB_{0,K,N}$ the set of all partitions of $\{1,\dots,N\}$ with cardinality between $0$ and $K$ inclusive i.e. it includes the empty-set.
From this, we obtain that DeepCluster is nothing else but
\begin{align}
    {\rm DeepCluster}=\min_{\theta \in \Theta} \min_{\mW \in \mathcal{W}_{\rm Kmeans}}\Tr\left(\mZ(\theta)^TL(\mW)\mZ(\theta)\right)
\end{align}


\subsection{NNCLR}

\begin{align}
    \mathcal{W}_{\rm Knn} \triangleq \left\{\sum_{n=1}^{N}\sum_{k\in \sB_k}\ve_n\ve_k^T+\ve_k\ve_n^T, \sB_n \in \mathcal{S}_{K}(N\setminus\{n\}),n=1,\dots,N \right\}
\end{align}

\begin{align}
    {\rm NNCLR}=\min_{\theta \in \Theta} \min_{\mW \in \mathcal{W}_{\rm 1nn}}\Tr\left(\mZ(\theta)^TL(\mW)\mZ(\theta)\right)
\end{align}
adding a predictor too ! leads to
\begin{align}
    {\rm MeanShift}=\min_{\theta \in \Theta} \min_{\mW \in \mathcal{W}_{\rm Knn}}\Tr\left(\mZ(\theta)^TL(\mW)\mZ(\theta)\right)
\end{align}


Furthermore, denoting the output of the projector as a function of the backbone's output $\mZ=\mU\mH$ we see that the VICReg formulation is instead equivalent to
\begin{align}
    \mathcal{L}=&\|\mU\mH^T\mH\mU^T-\mI\|_2^2+\Tr\left(\mU\mH^TL\mH\mU^T\right)\\
    =&\Tr(\mI)+\Tr(\mU^T\mU\mH^T\mH\mU^T\mU\mH^T\mH)-2\Tr(\mU\mH^T\mH\mU^T)+\Tr\left(\mU\mH^TL\mH\mU^T\right)\\
\end{align}
derivative is given by 
\begin{align}
    4\mH^T\mH\mU^T\mU\mH^T\mH\mU^T-2\mU\mH^T\mH +2\mU\mH^TL\mH 
\end{align}




\url{https://www.epfl.ch/labs/lts4/wp-content/uploads/2018/10/icassp2017b.pdf}

So $\mM$ defines a graph with $N$ nodes and the signal on the graph is given by the $N$ samples $\vz_n,n=1,\dots,N$. Again, the above can be expressed directly as 
\begin{align}
   \sum_{k=1}^{K}\max\left(0,1-\sqrt{Cov(\mZ)_{k,k}}\right)+ \|Cov(\mZ) \odot (\boldsymbol{1}-\mI) \|^2_{F}+\frac{1}{2}\|\underbrace{(\mI-\mM)}_{\text{Handmade Laplacian matrix}} \mZ\|_F^2.
\end{align}




so minimizing $\frac{1}{2}\|(\mI-\mM) \mZ\|_F^2$ means minimizing the diffusion process i.e. we want to minimize how much $\mZ$ diffuse to neighbors, with a $1$-step hop.

We can generalize this as follows
\begin{align}
   \sum_{k=1}^{K}\max\left(0,1-\sqrt{Cov(\mZ)_{k,k}}\right)+ \|Cov(\mZ) \odot (\boldsymbol{1}-\mI) \|^2_{F}+\frac{1}{2}\sum_{p=1}^{P}\|(\mI-\mM)^{p} \mZ\|_F^2,
\end{align}
but because we mostly connect pairs of nodes, we have that $(\mI-\mM)^{p}=p(\mI-\mM)$ and thus we can not exploit anything else from current hand-made graphs using only positive pairs.


GOAL1:{\bf introduce more positive samples per-batch + add an re-estimation procedure for $\mM$}.

Doing so, we will be able to leverage multi-hop diffusion process to further constrain the latent space "clustering".


GOAL2:{\bf leverage multi-hop relations $(\mI-\mM)^{p}$ in the loss}.

==> content/tikz_figures.tex <==


\begin{figure}[t!]
\centering
\begin{tikzpicture}[scale=0.17]

\pgfmathsetmacro{\height}{3}
\pgfmathsetmacro{\width}{8}
\pgfmathsetmacro{\leftOffset}{3}
\pgfmathsetmacro{\generalOffset}{0}

\volume{\generalOffset+ 10}{-2}{\generalOffset+10+\width}{2}

\Cvolume{\generalOffset+-\leftOffset}{2}{\generalOffset+-\leftOffset+\width}{3}{blue}
\Cvolume{\generalOffset+-\leftOffset}{-1}{\generalOffset+-\leftOffset+\width}{0}{blue}
\Cvolume{\generalOffset+10.05}{1.05}{\generalOffset+9.95+\width}{1.95}{blue}


\node[] at (\generalOffset+-\leftOffset+\width/2,1) {$\star$};

\draw [dashed] (\generalOffset+-\leftOffset+\width,3.1) -- (\generalOffset+10,2);
\draw [dashed] (\generalOffset+-\leftOffset+\width,-1.1) -- (\generalOffset+10,1);


\pgfmathsetmacro{\rightOffset}{4}

\Cvolume{\generalOffset+10+\width+\rightOffset}{1}{\generalOffset+10+2*\width+\rightOffset}{2}{black!30!green}
\Cvolume{\generalOffset+10+\width+\rightOffset}{-2}{\generalOffset+10+2*\width+\rightOffset}{-1}{black!30!green}
\Cvolume{\generalOffset+10.05}{-0.95}{\generalOffset+9.95+\width}{-0.05}{black!30!green}



\node[] at (\generalOffset+10+1.5*\width+\rightOffset,0) {$\star$};

\draw [dashed] (\generalOffset+10+\width + \rightOffset - 0.1,2.1) -- (\generalOffset+10+\width,0);
\draw [dashed] (\generalOffset+10+\width + \rightOffset - 0.1,-2.1) -- (\generalOffset+10+\width,-1);

\node[] at (37,+1) {$\text{multiplier=}2$};
\node[] at (37,-1) {$\text{factors=}2$};


\pgfmathsetmacro{\leftOffset}{3}
\pgfmathsetmacro{\generalOffset}{0}
\pgfmathsetmacro{\generalYOffset}{-8}

\volume{\generalOffset+ 10}{\generalYOffset+-2}{\generalOffset+10+\width}{\generalYOffset+2}

\Cvolume{\generalOffset+ 10-0.05}{\generalYOffset+1.05}{\generalOffset+9.95+\width}{\generalYOffset+2-0.05}{blue}
\Cvolume{\generalOffset+ 10}{\generalYOffset+-1+0.05}{\generalOffset+10+\width}{\generalYOffset-0.05}{black!30!green}


\Cvolume{\generalOffset+-\leftOffset}{\generalYOffset+2}{\generalOffset+-\leftOffset+\width}{\generalYOffset+3}{blue}
\Cvolume{\generalOffset+-\leftOffset}{\generalYOffset+-1}{\generalOffset+-\leftOffset+\width}{\generalYOffset+0}{blue}
\Cvolume{\generalOffset+-\leftOffset}{\generalYOffset+-4}{\generalOffset+-\leftOffset+\width}{\generalYOffset+-3}{blue}

\node[] at (\generalOffset+-\leftOffset+\width/2,\generalYOffset+1) {$\star$};
\node[] at (\generalOffset+-\leftOffset+\width/2,\generalYOffset+-2) {$\star$};


\draw [dashed] (\generalOffset+-\leftOffset+\width,\generalYOffset+3.1) -- (\generalOffset+10,\generalYOffset+2);
\draw [dashed] (\generalOffset+-\leftOffset+\width,\generalYOffset+-4.1) -- (\generalOffset+10,\generalYOffset+1);


\pgfmathsetmacro{\rightOffset}{4}

\Cvolume{\generalOffset+10+\width+\rightOffset}{\generalYOffset+1}{\generalOffset+10+2*\width+\rightOffset}{\generalYOffset+2}{black!30!green}
\Cvolume{\generalOffset+10+\width+\rightOffset}{\generalYOffset+-2}{\generalOffset+10+2*\width+\rightOffset}{\generalYOffset+-1}{black!30!green}
\Cvolume{\generalOffset+10+\width+\rightOffset}{\generalYOffset+-5}{\generalOffset+10+2*\width+\rightOffset}{\generalYOffset+-4}{black!30!green}

\node[] at (\generalOffset+10+1.5*\width+\rightOffset,\generalYOffset+0) {$\star$};
\node[] at (\generalOffset+10+1.5*\width+\rightOffset,\generalYOffset+-3) {$\star$};

\draw [dashed] (\generalOffset+10+\width + \rightOffset - 0.1,\generalYOffset+2.1) -- (\generalOffset+10+\width,\generalYOffset+0);
\draw [dashed] (\generalOffset+10+\width + \rightOffset - 0.1,\generalYOffset+-5.1) -- (\generalOffset+10+\width,\generalYOffset+-1);


\draw [] (\generalOffset-1,\generalYOffset+4.5) -- (\generalOffset+41,\generalYOffset+4.5);
\node[] at (\generalOffset+37,\generalYOffset-0.3) {$\text{multiplier=}3$};
\node[] at (\generalOffset+37,\generalYOffset-2.3) {$\text{factors=}3$};



\end{tikzpicture}
\vspace{-0.3cm}
    \caption{ Two LOST parametrizations of a conv1d layer with a single channel input making the layer weight a matrix of shape ({\rm n\_filters},{\rm filters\_length}). In {\bf both} cases, we use $K=R$ with value of $2$ as the {\bf top} and $3$ at the {\bf bottom} i.e. the resulting LOST layer has $2$ and $3$ times more parameters than the non over-parametrized counter-part. Note that padding is adjusted for the inter-filter convolutions to ensure that the final filter is of same length than the original layer. For multi-channel inputs, the same is applied to each of the ${\rm channels\_in}$ block of the conv1d layer weight.}
    \label{fig:codon1d}
\end{figure}

